Of Cores: A Partial-Exploration Framework for Markov Decision Processes

We introduce a framework for approximate analysis of Markov decision processes (MDP) with bounded-, unbounded-, and infinite-horizon properties. The main idea is to identify a "core" of an MDP, i.e., a subsystem where we provably remain with high probability, and to avoid computation on the less relevant rest of the state space. Although we identify the core using simulations and statistical techniques, it allows for rigorous error bounds in the analysis. Consequently, we obtain efficient analysis algorithms based on partial exploration for various settings, including the challenging case of strongly connected systems.

==> 0_macros.tex <==
\RequirePackage{xparse}
\RequirePackage{mathtools}
\RequirePackage{environ}
\RequirePackage{marvosym}

\usepackage{tikz}
\usetikzlibrary{automata,positioning,shapes,calc,fit,arrows.meta,backgrounds}
\usepackage{pgfplots}
\pgfplotsset{compat=1.13}

\colorlet{disabled}{lightgray}
\tikzstyle{state}=[draw,rectangle,inner sep=5pt,rounded corners=2pt]
\tikzstyle{action}=[font=\small,inner sep=0pt,outer sep=3pt]
\tikzstyle{actionnode}=[circle,draw=black,fill=black,minimum size=1mm,inner sep=0,outer sep=0]
\tikzstyle{actionedge}=[draw,-]
\tikzstyle{prob}=[font=\scriptsize,inner sep=0pt,outer sep=1pt]
\tikzstyle{probedge}=[draw,->]
\tikzstyle{directedge}=[draw,->]
\tikzset{chainarrow/.tip={Stealth[length=3pt]}}
\tikzset{>=chainarrow}



\DeclarePairedDelimiter{\delimabs}{\lvert}{\rvert}
\DeclarePairedDelimiter{\delimcardinality}{\lvert}{\rvert}
\DeclarePairedDelimiter{\delimset}{\lbrace}{\rbrace}
\DeclarePairedDelimiter{\delimtuple}{(}{)}

\NewDocumentCommand{\abs}{sm}{\IfBooleanTF{#1}{\delimabs{#2}}{\delimabs*{#2}}}
\NewDocumentCommand{\cardinality}{sm}{\IfBooleanTF{#1}{\delimcardinality{#2}}{\delimcardinality*{#2}}}
\NewDocumentCommand{\set}{sm}{\IfBooleanTF{#1}{\delimset{#2}}{\delimset*{#2}}}
\NewDocumentCommand{\tuple}{sm}{\IfBooleanTF{#1}{\delimtuple{#2}}{\delimtuple*{#2}}}


\newcommand{\powerset}[1]{\mathcal{P}(#1)}

\newcommand{\unionSym}{\cup}
\newcommand{\unionBin}{\mathbin{\unionSym}}
\newcommand{\strictunionSym}{\dot{\unionSym}}
\newcommand{\strictunionBin}{\mathbin{\dot{\unionSym}}}
\newcommand{\intersectionSym}{\cap}
\newcommand{\intersectionBin}{\mathbin{\intersectionSym}}
\newcommand{\UnionSym}{\bigcup}
\newcommand{\UnionBin}{\mathbin{\UnionSym}}
\newcommand{\strictUnionSym}{\dot{\UnionSym}}
\newcommand{\strictUnionBin}{\mathbin{\strictUnionSym}}
\newcommand{\IntersectionSym}{\bigcap}
\newcommand{\IntersectionBin}{\mathbin{\IntersectionSym}}

\newcommand{\union}{\unionBin}
\newcommand{\strictunion}{\strictunionBin}
\newcommand{\intersection}{\intersectionBin}
\newcommand{\Union}{\UnionSym}
\newcommand{\strictUnion}{\strictUnionSym}
\newcommand{\Intersection}{\IntersectionSym}

\newcommand{\Naturals}{\mathbb{N}}
\newcommand{\Reals}{\mathbb{R}}

\newcommand{\distribution}{p}
\NewDocumentCommand{\Distributions}{d()}{\IfNoValueTF{#1}{\mathcal{D}}{\mathcal{D}(#1)}}
\NewDocumentCommand{\Probability}{D[]{} D<>{} d[]}{
	\IfNoValueTF{#3}{\mathbb{P}_{#1}^{#2}}{\mathbb{P}_{#1}^{#2}\left[#3\right]}}
\NewDocumentCommand{\ProbabilityMax}{s D<>{} r[]}{\mathbb{P}^{\max}_{#2}\IfBooleanTF{#1}{\!\left[#3\right]}{[#3]}}
\NewDocumentCommand{\ProbabilityMin}{s D<>{} r[]}{\mathbb{P}^{\min}_{#2}\IfBooleanTF{#1}{\!\left[#3\right]}{[#3]}}
\NewDocumentCommand{\ProbabilityStrat}{D<>{\strategy} D<>{} d[]}{\mathbb{P}^{#1}_{#2}\IfNoValueTF{#3}{}{\left[#3\right]}}
\NewDocumentCommand{\Expectation}{D<>{} D<>{} d[]}{\IfNoValueTF{#1}{\mathbb{E}}{\mathbb{E}^{#1}_{#2}\left[#3\right]}}
\NewDocumentCommand{\ExpectationStrat}{D<>{\strategy} D<>{} d[]}{\mathbb{E}^{#1}_{#2}\IfNoValueTF{#3}{}{\left[#3\right]}}
\NewDocumentCommand{\integral}{m m}{\int #1\,d\,#2}
\NewDocumentCommand{\Sccs}{r()}{\mathsf{SCC}(#1)}
%\NewDocumentCommand{\Bsccs}{r()}{\mathsf{BSCC}(#1)}
\NewDocumentCommand{\Mecs}{r()}{\mathsf{MEC}(#1)}

%\NewDocumentCommand{\SuccessorExpectation}{d[]}{\IfNoValueTF{#1}{\mathbb{E}}{\mathbb{E}\left[#1\right]}}

\NewDocumentCommand{\reach}{d<>}{\IfNoValueTF{#1}{\Diamond}{\Diamond^{\leq #1}}}
\NewDocumentCommand{\always}{d<>}{\IfNoValueTF{#1}{\Box}{\Box^{\leq #1}}}
\newcommand{\true}{\mathsf{true}}
\newcommand{\false}{\mathsf{false}}

\newcommand{\MC}{\mathsf{M}}
\NewDocumentCommand{\mctransitions}{d()}{\IfNoValueTF{#1}{\delta}{\delta(#1)}}
\newcommand{\MDP}{\mathcal{M}}
\newcommand{\States}{S}
\newcommand{\initialstate}{s_0}
\newcommand{\Actions}{A}
\NewDocumentCommand{\stateactions}{d()}{\IfNoValueTF{#1}{\mathsf{Av}}{\mathsf{Av}(#1)}}
\NewDocumentCommand{\transitions}{d()}{\IfNoValueTF{#1}{\Delta}{\Delta(#1)}}
\newcommand{\infinitepath}{\rho}
\newcommand{\finitepath}{\varrho}
\newcommand{\strategy}{\pi}
\newcommand{\Strategies}{\Pi}
\newcommand{\StrategiesMD}{\Strategies^\mathsf{MD}}


\DeclareMathOperator{\support}{supp}


\NewDocumentCommand{\Core}{s t' D[]{\varepsilon}}{\IfBooleanTF{#1}
	{\overline{S}}{\IfBooleanTF{#2}{S'}{S}}_{#3}}
\NewDocumentCommand{\MinimalCore}{s t' D[]{\varepsilon}}{\IfBooleanTF{#1}{\overline{S}}{{\IfBooleanTF{#2}{S'}{S}}}_{#3}^\ast}
\NewDocumentCommand{\FiniteCore}{s t' D[]{\varepsilon} D<>{n}}{\IfBooleanTF{#1}
	{\overline{S}}{\IfBooleanTF{#2}{S'}{S}}_{#3, #4}}
\NewDocumentCommand{\MinimalFiniteCore}{s t' D[]{\varepsilon} D<>{n}}{\IfBooleanTF{#1}{\overline{S}}{{\IfBooleanTF{#2}{S'}{S}}}_{#3, #4}^\ast}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main.tex"
%%% End:

